Critical Evaluation of Deep Neural Networks for Wrist Fracture Detection

Wrist Fracture is the most common type of fracture with a high incidence rate. Conventional radiography (i.e. X-ray imaging) is used for wrist fracture detection routinely, but occasionally fracture delineation poses issues and an additional confirmation by computed tomography (CT) is needed for diagnosis. Recent advances in the field of Deep Learning (DL), a subfield of Artificial Intelligence (AI), have shown that wrist fracture detection can be automated using Convolutional Neural Networks. However, previous studies did not pay close attention to the difficult cases which can only be confirmed via CT imaging. In this study, we have developed and analyzed a state-of-the-art DL-based pipeline for wrist (distal radius) fracture detection -- DeepWrist, and evaluated it against one general population test set, and one challenging test set comprising only cases requiring confirmation by CT. Our results reveal that a typical state-of-the-art approach, such as DeepWrist, while having a near-perfect performance on the general independent test set, has a substantially lower performance on the challenging test set -- average precision of 0.99 (0.99-0.99) vs 0.64 (0.46-0.83), respectively. Similarly, the area under the ROC curve was of 0.99 (0.98-0.99) vs 0.84 (0.72-0.93), respectively. Our findings highlight the importance of a meticulous analysis of DL-based models before clinical use, and unearth the need for more challenging settings for testing medical AI systems.

==> tables/kappa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

\begin{table}[ht!]
\footnotesize
\centering

\begin{tabular}{C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.6cm}C{1.6cm}C{1.6cm}C{1.5cm}}
\toprule
    & \bfseries{Ground Truth} & \bfseries{Radiology Resident} & \bfseries{Radiologist \#1} & \bfseries{Radiologist \#2} & \bfseries{Primary Care Physician 1} & \bfseries{Primary Care Physician 2} & \bfseries{Primary Care Physician 3} & \bfseries{DeepWrist} \\ \midrule
Ground Truth                                                        & 1.0000          & 0.9274                                                        & 0.9793        & 0.9897        & 0.7616                                                              & 0.8790                                                              & 0.6296                                                              & 0.8848    \\ \hline
\begin{tabular}[c]{@{}c@{}}Radiology \\ Resident\end{tabular}       &              & 1.0000                                                           & 0.9270        & 0.9380        & 0.7252                                                              & 0.848                                                               & 0.6338                                                              & 0.8519    \\ \hline
Radiologist 1                                                       &              &                                                               & 1.0000           & 0.9691        & 0.7593                                                              & 0.8584                                                              & 0.6476                                                              & 0.8840    \\ \hline
Radiologist 2                                                       &              &                                                               &               & 1.0000           & 0.7520                                                              & 0.8893                                                              & 0.6208                                                              & 0.8747    \\ \hline
\begin{tabular}[c]{@{}c@{}}Primary Care \\ Physician 1\end{tabular} &              &                                                               &               &               & 1.0000                                                                 & 0.6660                                                              & 0.5500                                                              & 0.6749    \\ \hline
\begin{tabular}[c]{@{}c@{}}Primary Care \\ Physician 2\end{tabular} &              &                                                               &               &               &                                                                     & 1.0000                                                                 & 0.5620                                                              & 0.7857    \\ \hline
\begin{tabular}[c]{@{}c@{}}Primary Care \\ Physician 3\end{tabular} &              &                                                               &               &               &                                                                     &                                                                     & 1.0000                                                                 & 0.6711    \\ \hline
DeepWrist                                                           &              &                                                               &               &               &                                                                     &                                                                     &                                                                     & 1.0000       \\ \bottomrule
\end{tabular}
\caption{Cohen's Quadratic Kappa: Inter-Reader Agreement analysis}
\label{tab:kappa}
\end{table}
